New Methods to Improve Large-Scale Microscopy Image Analysis with Prior Knowledge and Uncertainty

Multidimensional imaging techniques provide powerful ways to examine various kinds of scientific questions. The routinely produced datasets in the terabyte-range, however, can hardly be analyzed manually and require an extensive use of automated image analysis. The present thesis introduces a new concept for the estimation and propagation of uncertainty involved in image analysis operators and new segmentation algorithms that are suitable for terabyte-scale analyses of 3D+t microscopy images.

==> Content/0_Abstracts/Erklaerung.tex <==


\selectlanguage{ngerman}
\addcontentsline{toc}{chapter}{Selbstst\"andigkeitserkl\"arung} 

\chapter*{Selbstst\"andigkeitserkl\"arung}
Hiermit erkl\"are ich, Johannes Stegmaier, dass ich die vorliegende Arbeit selbst-st\"andig angefertigt und keine anderen als die angegebenen Quellen und Hilfsmittel benutzt sowie die w\"ortlich und inhaltlich \"ubernommenen Stellen als solche kenntlich gemacht und die Satzung der Universit\"at Karlsruhe (TH) zur Sicherung guter wissenschaftlicher Praxis in der jeweils g\"ultigen Fassung beachtet habe.

\begin{center}
\parbox{4.5cm}{\vspace{1cm}Karlsruhe, {\today}\hrule
\strut \footnotesize Ort, Datum} \hfill\parbox{4cm}{\includegraphics[scale=0.6]{SignatureBlank}\hrule
\strut \footnotesize Johannes Stegmaier}
\end{center}

\selectlanguage{american}


==> Content/1_Introduction/BiologicalBackground.tex <==
%!TEX root = ../Dissertation.tex

%%%%%%%%%%%%%%%%%%%%%%% RESULTS %%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Results and Discussion}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% BENCHMARKING %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Benchmarks}

\begin{table*}[htb]
\begin{center}
\begin{tabular}{lcccccccc}
\toprule
{Name} & {URL} & {JI} & {Hausdorff} & NSD ($\times$10) & Split & Merged & Spurious & Missing \\
\midrule
%	\texttt{http://pacific.mpi-cbg.de/wiki/index.php/SPIM_Registration}
\bottomrule
\end{tabular}
\end{center}
\end{table*}

\begin{itemize}
	\item Implement the methods mentioned in \cite{Coelho09} in Gait-CAD
	\item define a measure to quantify the quality of detected seeds (distance to nearest neighbor within range, does nearest neighbor in the range exist at all?)
	\item A biosegmentation benchmark for evaluation of bioimage analysis methods --> contains measure for detected seeds combined with regions.
	
	\item software for gradient vector flow http://www.biomedcentral.com/1471-2121/8/40

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%% BIOLOGICAL BACKGROUND %%%%%%%%%%%%%%%%%%%%%%%%
\section{Biological Background}


%%%%%%%%%%%%%%%%%%%%%%% DEVELOPMENTAL BIOLOGY %%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Developmental Biology}

The cycle of life:
\begin{itemize}
	\item Fertilization: Mature sex cells (sperm, egg, also known as gametes) fusionate and combine their their chromosomes (only half of the full chromosome amount) to build the whole genome of the organism.
	\item Cleavage: Rapid division of the fertilized egg into smaller cells, known as blastomeres. Blastomeres rearrange and build the blastula, a sphere of cells.
	\item Mitotic division slows down and blastomeres move their relative positions. This process is known as gastrulation, i.e. the embryo is said to be in the gastrula stage of development.
	\item During the so called organogenesis cells rearrange and interact with each other, forming tissue and organs.
	\item \cite{Gilbert10}
\end{itemize}

At the end of gastrulation the following regions with the respective precursor cells have formed:

Ectoderm: Outer cell layer that encloses the entire embryo. Consists of precursor cells that later on form the epidermis, the brain and the nerves.

Endoderm: Is located on the inside of the embryo and contains the precursor cells for the gut and the respiratory systems.

Mesoderm: Located between endoderm and ectoderm, forming the connective tissue, blood, heart, skeleton, gonads and kidneys at later states.

Epidermis: cell layer forming the skin of an organism

\subsection{Zebrafish}

\cite{Esch12} Mini review about Zebrafish as a model organism for developmental invesigation.



%%%%%%%%%%%%%%%%%%%%%%% MICROSCOPY %%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Microscopy}


%%%%%%%%%%%%%%%%%% COMPOUND MICROSCOPY %%%%%%%%%%%%%%%%%%%%
\subsubsection{Compound Microscopy}


%%%%%%%%%%%%%%%%%%%%%%% SPIM %%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{SPIM - Single Plane Illumination Microscopy}
\begin{itemize}
	\item \cite{Huisken04, Huisken09}: First paper that describes SPIM and applies the technique to live embryo microscopy.
	
	\item \cite{Keller11a}: Provide an overview of the history of light sheet
microscopy, review the development of tissue clearing
methods, and discuss recent technical breakthroughs that
have the potential to influence the future direction of the field.
	
	- Modern life science research often requires multidimensional imaging of a complete spatiotemporal pattern of gene and protein expression or tracking of tissues during the development of an intact embryo (1)
	
	- 
	\item \cite{Weber11} (Light sheet microscopy for real-time developmental biology, add to biosignal.bib): Review over the current SPIM technology, including theoretical background etc.
	
	\item \cite{Krzic12} (Multiview light-sheet microscope for rapid in toto imaging): Use 2 cameras that are placed opposite to one another and two light sheet laser generators placed in 90 degree angles from the cameras. Image ackquisition is performed successively for each camera combined with each light sheet, ending up with four images. Due to possible misalignment of camera arms, smaller rotation of embryo or not perfectly aligned setup, scaling for mismatched magnifications. To cope with this fact, the four images are registered using a affine transformation for which the parameters are estimated only once in the beginning and remain the same for the given setup --> Speedup of the registration as only a known transformation has to be applied. Parameters are refined after some hours of ackquisition. Weighted average is used for the image fusion, where good regions are weighted stronger than weaker ones. Use 2560x2160x101 resolution. Use maximum likelihood deconvolution with the known PSF of the microscope. Use 2 QuadCore Xeon CPU with 48Gb ram and ITK. MATLAB is used for image synthesis and bead analysis. Use local thresholding and subsequent watershed for the segmentation.
	
	\item Not Read Yet: \cite{Tomer11, Megason03}
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%% DSLM %%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{DSLM - Digital Scanned Laser Light Sheet Fluorescence Microscopy}

\begin{itemize}
	\item \cite{Keller08SC}: 
	- \textit{SPIM - Single Plane Illumination Microscopy} genereates 3D images with reduced energy load on the specimen. Light sheet illuminates slices of the sample and fluorescence is captured by a CCD. \
	
	- \textit{Digital scanned laser light sheet fluorescence microscopy (DSLM)}, has higher spatio-temporal resolution, signal-to-noise ratio and is therefore better suited for imaging of whole embryo cell lineages (in this case: Zebrafish image resolution of 2048x2048x400 resolution and t = 60-90s). mRNA injection of H2Be-GFP at one-cell-level, which binds to chromatin and therefore allows to track the nuclei. --> ended up with 400k images of the embryo. \
	
	- employ heavily parallelized algorithms to further process the large amount of data (Used Matlab).
	
	--> For segmentation of the cell nuclei: recursive refinement, filtering according to nuclei specific morphological properties (\textit{a priori} knowledge attained by analyzing nuclei at a specific developmental stage). Method only works well for high SNR and high Dynamic Range (14Bit in this case))
	
	--> Tracking by nearest-neighbor search.
		
	--> Rest of the paper is the biological explanation of the cell behavior.
	
	--> Related Articles:
		Keller et al., 2011: Digital scanned laser light-sheet fluorescence microscopy (DSLM) of zebrafish and Drosophila embryonic development.
		Fast, high-contrast imaging of animal development with scanned light sheet-based structured-illumination microscopy \cite{Keller11}
		
		\item Landmarks in the images are performed using the following TetraSpeck microspheres \url{http://www.invitrogen.com/1/1/11129-tetraspeck-microspheres-0-5-\%CE\%BCm-fluorescent-blue-green-orange-dark-red.html}
		
		\end{itemize}
		

==> Content/2_UncertaintyFramework/UncertaintyApplications.tex <==

%%%%%%%%%%%%%%%%%%% UNCERTAINTY ESTIMATION AND PROPAGATION %%%%%%%%%%%%%%%%%%%
\section{Potential Applications of the Uncertainty Framework}

\subsection{Uncertainty-based Information Fusion}
\label{sec:chap2:FeatureFusion}

\subsection{Using Membership Degree for Object Rejection}
In the case of improper image material, the quality of information extracted by automated processing operators is often limited. A primary goal of automated processing should be keeping the number of true positives large and the number of false negatives small. In some cases, such as the detection of a moving target, it is crucial to reliably detect it. Hence, it is sometimes necessary to use parameter values that on the one hand reliably detect all desired objects in the image while on the other hand also detecting many false positives that correspond to noise or image artifacts. Based on the previously described prior knowledge formulation it is possible to exploit extracted features for a coarse classification based on fuzzy set membership association. Here, it should be focused on a binary classification problem, i.e., if an extracted object corresponds either to the desired class or to the undesired class that can be discarded.

In the case of volumetric image data by intuition one would apply 3D pendants of 2D algorithms. This choice is definitely reasonable in most cases. However, the application of explicit 3D algorithms might become infeasible due to the required resources or if they yield poor results due to illumination variations in sequentially recorded image stacks. An approach to tackle this problem is the use of 2D algorithms on each of the available slices and to perform a fusion of the extracted features afterwards. Of course, it is mandatory to have a strong knowledge about the expected outcome in order to perform a reproducible and quality increasing feature fusion.

\subsection{}

%%%%%%% FEATURE FUSION %%%%%%%

\subsection{Fusion of Extracted Features}
\label{sec:chap2:FusionOfExtractedFeatures}
Besides performing the fusion directly on the image material it can also be performed on extracted feature values. This becomes especially interesting if the content of rotationary complement images cannot be fused reliably due to strong changes of the investigated probe. For instance, depending on the image resolution (both axial and lateral), the time needed by the stepper motors to rotate the specimen, as well as limitations of the acquisition speed provided by the microscope, several seconds up to a few minutes are required to capture a single image stack. During this relatively low sampling rate, it has to be considered that cells in a developing organism may migrate, divide or die during the acquisition period unless the time resolution of acquired images is sufficiently high. 



\begin{itemize}
	\item \cite{Pohl98}: Review about multi sensor image fusion. Describe for example the different levels of image fusion (pixel level, feature level, decision level). Focus however lies on the pixel level.
	\item \cite{Vazquez-Reina11}: Fusion of 2D Segmentation results of brain slices.
\end{itemize}


\begin{figure}[htb]
\centerline{\includegraphics[width=\columnwidth]{Figures/2_UncertaintyFramework/UncertaintyBasedFusion/SeedFusionCases.png}}

\caption[Possible cases for seed point fusion]{Possible cases for seed point fusion: spheres are touching (A), one centroid inside the other sphere (B), centroid of bigger sphere inside the smaller sphere (C), smaller sphere completely within the larger sphere (D), percentual amount of overlap (E). Depending on the fusion task, different approaches might be considered.}
\label{fig:SeedFusionCases}
\end{figure}

\begin{table}[htb]
	\centering
	\rowcolors{2}{white}{gray!25}
	\begin{tabular}{lll}
		\toprule
		\textbf{Description} 		& \textbf{Case} & \textbf{Formula} \\
		\midrule
		Spheres are touching    & A & $d \leq r_1+r_2$ \\
		One centroid inside the oder sphere    & B & $d \leq \max \left(r_1,r_2 \right)$ \\
		Centroid of bigger sphere inside smaller sphere   & C & $d \leq \min \left(r_1,r_2 \right)$ \\
		One Sphere completely within other sphere    & D & $d \leq \left| r_1-r_2 \right|$ \\
		Thresholded procentual amount of overlap    & E & $V_{\text{thres}} \leq \frac{\frac{\pi}{3} \left[h_1^2 \cdot (3r_1-h_1) + h_2^2 \cdot (3r_2-h_2) \right]}{V_1+V_2}$ \\
			
		\bottomrule
	\end{tabular}
	
	\caption{Different cases for the fusion of bounding spheres. The cases refer to the drawings depicted in \cref{fig:SeedFusionCases}.}
	\label{tab:Chapter5_WorstCaseComplexityAnalysis}
\end{table}


In addition, determining a threshold on the estimated uncertainty values with a fixed value range of $[0,1]$ is more intuitive than directly using a single feature-based threshold that might have different feasible ranges for each feature. Down-stream processing operators benefit from this rough classification of extracted information, as they do not have to take care of different parameter ranges but can operate on a dimensionless quantity with known range. Furthermore, instead of a binary decision, the gradual membership to the set of 


==> Content/4_AlgorithmEnhancement/CompletePipeline.tex <==


\section{Enhancing a Comprehensive Pipeline with Uncertainty Propagation}

\subsection{Validation}

\begin{itemize}
	\item perform the processing on the simulated benchmark for a pipeline with and without uncertainty processing. 
	\item compare speed and check if the uncertainty handling drastically increases memory or processing times
	\item use the pipeline evaluation measure developed in the benchmark chapter for evaluation.
\end{itemize}


==> preface.tex <==
\title{New Methods to Improve Large-Scale Microscopy Image Analysis with Prior Knowledge and Uncertainty}

\subtitle{
	{\Large }
	\vskip 15mm
	{\normalsize \textmd{
	Zur Erlangung des akademischen Grades eines\\ 
	Doktors der Ingenieurwissenschaften\\
	(Dr.-Ing.)\\
	\vskip 5mm
	bei der Fakult\"at f\"ur Maschinenbau\\ 
	des Karlsruher Instituts f\"ur Technologie (KIT)\\
	\vskip 15mm
	% eingereichte\\
	genehmigte\\
	DISSERTATION
	}}
	\vskip 5mm
}

\author{
	{\normalsize \sffamily von}\\
	{\Large \sffamily M.Sc. Johannes Stegmaier}
}

\date{}

\publishers{
	\vskip 25mm
	{\small \sffamily
	\begin{tabular}{ll}
 		Datum der m\"undlichen Pr\"ufung: & 03. Juni 2016 \\
 		Referent:      & apl. Prof. Dr.-Ing. Ralf Mikut \\
 		Korreferenten: &Prof. Dr. Uwe Str\"ahle \\
									 &Prof. Dr. Jan. G. Korvink \\
	\end{tabular}
	}
}

